The Star Formation Reference Survey. II. Activity demographics and host-galaxy properties for Infrared-selected galaxies

We present activity demographics and host-galaxy properties of infrared-selected galaxies in the local Universe, using the representative Star Formation Reference Survey (SFRS). Our classification scheme is based on a combination of optical emission-line diagrams (BPT) and IR-color diagnostics. Using the weights assigned to the SFRS galaxies based on its parent sample, a far-infrared-selected sample comprises 71\% H\,\textsc{ii} galaxies, 13\% Seyferts, 3\% Transition Objects (TOs), and 13\% Low-Ionization Nuclear Emission-Line Regions (LINERs). For the SFRS H\,\textsc{ii} galaxies we derive nuclear star-formation rates and gas-phase metallicities. We measure host-galaxy metallicities for all galaxies with available long-slit spectroscopy and abundance gradients for a subset of 12 face-on galaxies. The majority of H\,\textsc{ii} galaxies show a narrow range of metallicities, close to solar, and flat metallicity profiles. Based on their host-galaxy and nuclear properties, the dominant ionizing source in the far-infrared selected TOs is star-forming activity. LINERs are found mostly in massive hosts (median of $10^{10.5}$ M$_{\odot} $), median $L(60\mu m) = 10^{9}$ L$_{\odot}$, median dust temperatures of $ F60/F100 = 0.36 $, and median $L_{\textrm{H}\alpha}$ surface density of $ 10^{40.2} $ erg s$ ^{-1} $kpc$ ^{-2} $, indicating older stellar populations as their main ionizing source rather than AGN activity.

==> Source files/Activity_Classification_Table_v3_10lines.tex <==
\begin{table*}
      \begin{minipage}{142mm}
\caption{Activity classification based on different diagnostics. Column (1) SFRS ID (\citealt{SFRS}); Column (2) Galaxy name; Columns (3) - (5) present the nuclear activity classification of the three diagnostic BPT diagrams. Column (6) shows the IRAC color classification based on both the nuclear and integrated colors. Columns (7) and (8) present the MEx and CEx diagrams classification, and Column (9) presents the final adopted classification based on the combination of the three BPT diagnostics and the IRAC color--color diagram. Broad-line (Type-1) Sy and LINERs are reported as Sy-1 and LINER-1 respectively, otherwise Type-2 AGNs are implied. The full version of Table \ref{table2} is available online from MNRAS.} 
	\label{table2}
	\begin{tabular}{@{}ccccccccc}
 \hline
 
 SFRS & Galaxy & \multicolumn{3}{c}{Nuclear Spectra BPT} & IRAC Colors & MEx & CEx & Final Classification \\
\multicolumn{2}{c}{} & [N\,{\sc ii}]/H$\alpha$ & [S\,{\sc ii}]/H$\alpha$ & [O\,{\sc i}]/H$\alpha$ & & & \\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\
 \hline
  1 & IC~486 & Sy & Sy & Sy & Sy & Sy & Sy & Sy\\
2 & IC~2217 & HII & HII & HII & HII & HII & HII & HII\\
3 & NGC~2500 & TO & LINER & LINER & HII & HII & \ldots & LINER\\
4 & NGC~2512 & HII & HII & HII & HII & HII & \ldots & HII\\
5 & MCG~6-18-009 & HII & HII & HII & HII & HII & HII & HII\\
6 & MK~1212 & TO & HII & HII & HII & HII & HII & HII\\
7 & IRAS~08072+1847 & TO & HII & HII & Sy & HII & TO & Sy\\
8 & NGC~2532 & HII & HII & HII & \ldots & HII & HII & HII\\
9 & UGC~4261 & HII & HII & HII & HII & TO & HII & HII\\
10 & NGC~2535 & HII & HII & HII & HII & HII & \ldots & HII\\
 \hline
	\end{tabular}

\end{minipage}
\end{table*}



==> Source files/DEW_v5a.tex <==
\begin{table*}
%	\begin{minipage}{120mm}
		        \caption{SED characteristic of the ``reference" galaxies generated with CIGALE, and EW differences between ``reference" and ``model" spectra. Columns (1) - (2) The age of the onset of star formation in Myrs and the E($ B-V $), describing the star-formation history and color excess of the generated ``reference" SEDs; Column (3) - (4) The EW of the H$ \beta $ and H$ \alpha $ absorption lines for the ``reference" spectra; Columns (5) - (6) The mean and standard deviation of the difference of the EW(H$ \beta $) for each of the ``model" spectra from their corresponding ``reference" spectrum (see Section \ref{Balmer-test}); Columns (7) - (8) Similar to Columns (5) and (6) for the EW(H$ \alpha $). All EWs and $\langle \Delta EW\rangle$ values are given in units of \AA.}
		\label{Balmer-Table}
                \hspace*{-1.1cm}\begin{tabular}{@{}cccccccc}
			\hline
Age & $E( B-V $) & $EW_{H \beta}$ & $EW_{H \alpha}$ & $\langle \Delta EW_{H \beta}\rangle$ & $\sigma_{\Delta EW_{H\beta}} $ & $\langle \Delta EW_{H \alpha}\rangle$ & $\sigma_{\Delta EW_{H\alpha}} $ \\
           (Myr) & (mag) & (Ref) & (Ref) & (Mod--Ref) & (Mod--Ref) & (Mod--Ref) & (Mod--Ref)\\            
			(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
			\hline

  50 & 0.16 & 3.89 & 2.42 & 0.30 & 0.12 & 0.16 & 0.06\\
  50 & 0.32 & 3.97 & 2.45 & 0.23 & 0.11 & 0.12 & 0.05\\
  50 & 0.65 & 4.09 & 2.48 & 0.11 & 0.10 & 0.06 & 0.05\\
  100 & 0.16 & 4.92 & 2.92 & 0.18 & 0.13 & 0.11 & 0.06\\
  100 & 0.32 & 5.08 & 2.98 & 0.16 & 0.10 & 0.09 & 0.05\\
  100 & 0.65 & 5.25 & 3.05 & 0.08 & 0.10 & 0.04 & 0.04\\
  200 & 0.16 & 6.85 & 3.84 & $-$0.06 & 0.11 & 0.03 & 0.04\\
  200 & 0.32 & 6.98 & 3.89 & $-$0.01 & 0.11 & 0.04 & 0.04\\
  200 & 0.65 & 7.08 & 3.94 & 0.01 & 0.09 & 0.02 & 0.04\\
  400 & 0.16 & 9.39 & 4.75 & $-$0.09 & 0.07 & $-$0.02 & 0.04\\
  400 & 0.32 & 9.41 & 4.75 & $-$0.09 & 0.06 & $-$0.01 & 0.04\\
  400 & 0.65 & 9.42 & 4.76 & $-$0.09 & 0.07 & $-$0.02 & 0.04\\
  500 & 0.16 & 9.57 & 4.77 & $-$0.15 & 0.02 & $-$0.05 & 0.02\\
  500 & 0.32 & 9.57 & 4.77 & $-$0.15 & 0.03 & $-$0.05 & 0.02\\
  500 & 0.65 & 9.58 & 4.77 & $-$0.16 & 0.02 & $-$0.05 & 0.02\\
  1000 & 0.16 & 6.52 & 3.71 & $-$0.06 & 0.06 & $-$0.01 & 0.03\\
  1000 & 0.32 & 6.52 & 3.71 & $-$0.05 & 0.06 & $-$0.01 & 0.03\\
  1000 & 0.65 & 6.52 & 3.71 & $-$0.06 & 0.05 & $-$0.01 & 0.03\\
  1500 & 0.16 & 4.65 & 3.10 & $-$0.06 & 0.05 & $-$0.03 & 0.03\\
  1500 & 0.32 & 4.65 & 3.10 & $-$0.06 & 0.06 & $-$0.03 & 0.03\\
  1500 & 0.65 & 4.65 & 3.10 & $-$0.06 & 0.05 & $-$0.03 & 0.03\\
  2000 & 0.16 & 3.95 & 2.82 & $-$0.18 & 0.07 & $-$0.07 & 0.02\\
  2000 & 0.32 & 3.95 & 2.82 & $-$0.18 & 0.05 & $-$0.07 & 0.02\\
  2000 & 0.65 & 3.95 & 2.82 & $-$0.15 & 0.06 & $-$0.06 & 0.02\\
\hline
        \end{tabular}

%\end{minipage}
\end{table*}


==> Source files/Line_Ratios_Table_v6_10lines.tex <==
%\begin{landscape}

\begin{table*}
\begin{scriptsize}

	\hspace*{-0.9cm}\begin{minipage}{194mm}
	\caption{Nuclear fluxes and flux ratios of optical diagnostic emission lines. Column (1) SFRS ID (\citealt{SFRS}); Column (2) Galaxy name; Column (3) H$\alpha$ emission line flux, normalized to 10$^{-14}$ erg cm$^{-2}$ s$^{-1}$; Column (4) Ratio of H$\alpha$ and H$\beta$ Balmer line fluxes. Columns (5) $-$ (8) BPT line ratio measurements and uncertainties; Column (9) Extinction corrected H$\alpha$ emission line flux normalized to 10$^{-14}$ erg cm$^{-2}$ s$^{-1}$; Columns (10) and (11) Integrated and nuclear extinction as calculated by $\textsc{starlight}$ code; Column (12) The nuclear E(B-V) color excess of the gas as calculated from the Balmer decrement; Column (13) Spectral observation method. Emission line fluxes and ratios for the FAST observations come from the nuclear aperture spectrum. F(H$\alpha$)$_{cor}$ and E(B-V)$_{\textrm{gas}} $ values flagged with a * symbol indicate uncertain measurements due to differences in the flux calibration between the blue and red spectral regions of galaxies observed with the 600 l mm$^{-1}$ grating configuration (Section \ref{FAST-SDSS}). The full version of Table \ref{table1} is available online from MNRAS.} 
	\label{table1}
	{\renewcommand{\arraystretch}{1.35}
	\begin{tabular}{@{}ccccccccccccc}
 \hline
SFRS & Galaxy & F(H$\alpha$) & H$\alpha$/H$\beta$ & [O\,{\sc iii}]/H$\beta$ & [N\,{\sc ii}]/H$\alpha$ & [S\,{\sc ii}]/H$\alpha$ & [O\,{\sc i}]/H$\alpha$ & F(H$\alpha$)$_{cor}$ & A$_{V}$ & A$_{V}\textrm{nuc}$ & E(B-V)$ _{\textrm{gas}} $ & Observation \\
 (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
 \hline

1 & IC~486 & 2.430$\substack{+0.037 \\ -0.026}$ & 5.830$\substack{+0.214 \\ -0.205}$ & 1.058$\substack{+0.015 \\ -0.015}$ & 0.071$\substack{+0.006 \\ -0.008}$ & -0.105$\substack{+0.005 \\ -0.007}$ & -0.727$\substack{+0.019 \\ -0.020}$ & 10.788$\substack{+0.164 \\ -0.115}$ & \ldots & 0.68 & 0.64 & SDSS \\ 
2 & IC~2217 & 7.660$\substack{+0.045 \\ -0.045}$ & 4.935$\substack{+0.085 \\ -0.087}$ & -0.552$\substack{+0.029 \\ -0.029}$ & -0.422$\substack{+0.006 \\ -0.006}$ & -0.474$\substack{+0.003 \\ -0.003}$ & -1.588$\substack{+0.052 \\ -0.054}$ & 27.755$\substack{+0.163 \\ -0.163}$ & 0.50 & 0.82 & 0.55 & FAST \\ 
3 & NGC~2500 & 0.151$\substack{+0.007 \\ -0.007}$ & 3.096$\substack{+0.497 \\ -0.482}$ & 0.132$\substack{+0.080 \\ -0.083}$ & -0.446$\substack{+0.057 \\ -0.058}$ & -0.268$\substack{+0.022 \\ -0.019}$ & 0.127$\substack{+0.031 \\ -0.029}$ & 0.182$\substack{+0.008 \\ -0.008}$ & 0.81 & 0.68 & 0.08 & FAST \\ 
4 & NGC~2512 & 10.800$\substack{+0.008 \\ -0.008}$ & 4.713$\substack{+0.017 \\ -0.017}$ & -0.677$\substack{+0.008 \\ -0.008}$ & -0.310$\substack{+0.001 \\ -0.001}$ & -0.564$\substack{+0.002 \\ -0.002}$ & -1.535$\substack{+0.014 \\ -0.014}$ & 35.104$\substack{+0.026 \\ -0.026}$ & 0.52 & 0.46 & 0.50 & FAST \\ 
5 & MCG~6-18-009 & 6.230$\substack{+0.041 \\ -0.041}$ & 5.253$\substack{+0.075 \\ -0.072}$ & -0.517$\substack{+0.015 \\ -0.014}$ & -0.289$\substack{+0.004 \\ -0.004}$ & -0.564$\substack{+0.003 \\ -0.003}$ & -1.441$\substack{+0.023 \\ -0.024}$ & 26.157$\substack{+0.172 \\ -0.172}$ & \ldots & 0.63 & 0.61 & SDSS \\ 
6 & MK~1212 & 0.403$\substack{+0.005 \\ -0.004}$ & 6.165$\substack{+0.323 \\ -0.318}$ & -0.316$\substack{+0.054 \\ -0.049}$ & -0.285$\substack{+0.009 \\ -0.008}$ & -0.562$\substack{+0.005 \\ -0.005}$ & -1.441$\substack{+0.053 \\ -0.072}$ & 2.469$\substack{+0.031 \\ -0.025}$ & \ldots & 0.94 & 0.78 & SDSS \\ 
7 & IRAS~08072+1847 & 1.790$\substack{+0.013 \\ -0.013}$ & 8.168$\substack{+0.165 \\ -0.160}$ & -0.239$\substack{+0.020 \\ -0.018}$ & -0.196$\substack{+0.005 \\ -0.005}$ & -0.469$\substack{+0.003 \\ -0.003}$ & -1.187$\substack{+0.023 \\ -0.021}$ & 17.611$\substack{+0.128 \\ -0.128}$ & \ldots & 1.51 & 0.98 & SDSS \\ 
8 & NGC~2532 & 2.300$\substack{+0.060 \\ -0.056}$ & 7.691$\substack{+1.296 \\ -1.221}$ & -0.519$\substack{+0.068 \\ -0.072}$ & -0.415$\substack{+0.028 \\ -0.030}$ & -0.492$\substack{+0.010 \\ -0.011}$ & -1.693$\substack{+0.010 \\ -0.011}$ & 23.745$\substack{+0.619 \\ -0.578}$ & 0.53 & 0.79 & 1.00 & FAST \\ 
9 & UGC~4261 & 8.290$\substack{+0.043 \\ -0.043}$ & 4.195$\substack{+0.039 \\ -0.040}$ & 0.014$\substack{+0.005 \\ -0.005}$ & -0.597$\substack{+0.004 \\ -0.004}$ & -0.591$\substack{+0.002 \\ -0.002}$ & -1.690$\substack{+0.012 \\ -0.012}$ & 20.472$\substack{+0.106 \\ -0.106}$ & \ldots & 0.49 & 0.39 & SDSS \\ 
10 & NGC~2535 & 2.310$\substack{+0.013 \\ -0.013}$ & 4.137$\substack{+0.089 \\ -0.092}$ & -0.885$\substack{+0.077 \\ -0.072}$ & -0.434$\substack{+0.007 \\ -0.007}$ & -0.614$\substack{+0.002 \\ -0.002}$ & -1.741$\substack{+0.163 \\ -0.257}$ & 5.520$\substack{+0.031 \\ -0.031}$ & 0.65 & 0.48 & 0.37 & FAST \\ 

\hline
	\end{tabular}
	}

\end{minipage}
\end{scriptsize}
\end{table*}

%\end{landscape}



==> Source files/Probabilistic_AC_Table_v2_10lines.tex <==
\begin{table*}
      \begin{minipage}{140mm}
	\caption{Probabilistic activity classification types based on the uncertainties of line measurements and following the methods outlined in Section \ref{Prob-AC}. The full version of Table \ref{Prob-AC} is available online from MNRAS.}
	\label{Prob-AC}
	\begin{tabular}{@{}ccccccccccc}
 \hline
 SFRS & Galaxy & \multicolumn{3}{c}{[N\,{\sc ii}]/H$\alpha$} & \multicolumn{3}{c}{[S\,{\sc ii}]/H$\alpha$} & \multicolumn{3}{c}{[O\,{\sc i}]/H$\alpha$} \\
\multicolumn{2}{c}{} & H\,{\sc ii} & TO & Sy / LINER & H\,{\sc ii} & LINER & Sy & H\,{\sc ii} & LINER & Sy \\
 \hline  
1 & IC~486 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 \\ 
2 & IC~2217 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
3 & NGC~2500 & 0.334 & 0.666 & 0.000 & 0.326 & 0.573 & 0.101 & 0.000 & 1.000 & 0.000 \\ 
4 & NGC~2512 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
5 & MCG~6-18-009 & 0.729 & 0.271 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
6 & MK~1212 & 0.000 & 1.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
7 & IRAS~08072+1847 & 0.000 & 1.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
8 & NGC~2532 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
9 & UGC~4261 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
10 & NGC~2535 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 \\ 
 \hline
	\end{tabular}

\end{minipage}
\end{table*}



==> Source files/Z-tables_v2.tex <==

\begin{landscape}

\begin{table}
	\begin{minipage}{136mm}
		\begin{center}
			
	\caption{Host galaxy and nuclear metallicities and SFRs for the SFRS SFGs. Host-galaxy metallicities are given only for galaxies observed with long-slit spectroscopy, with their nuclear contribution subtracted. SFR values flagged with a * symbol indicate uncertain measurements due to differences in the flux calibration between the blue and red spectral regions of galaxies observed with the 600 l mm$^{-1}$ grating configuration (Section \ref{FAST-SDSS}). The full version of Table \ref{Nuc-Host-Z-SFR} is available online from MNRAS.} 
	\label{Nuc-Host-Z-SFR}
	\begin{tabular}{@{}ccccccc}

 \hline
 SFRS & Galaxy & \multicolumn{2}{c}{Nuclear Metallicity} & \multicolumn{2}{c}{Host Galaxy Metallicity} & $\log\textrm{SFR}$\\
\multicolumn{2}{c}{} & O3N2 & N2 & O3N2 & N2 & (Nuclear) \\ 
 \hline
 2 & IC~2217 & 8.772 $\pm$ 0.009 & 8.659 $\pm$ 0.003 & 8.717 $\pm$ 0.011 & 8.941 $\pm$ 0.004 & 0.014 $\pm$ 0.003\\
 4 & NGC~2512 & 8.847 $\pm$ 0.002 & 8.723 $\pm$ 0.001 & 8.743 $\pm$ 0.013 & 8.909 $\pm$ 0.003 & 0.035 $\pm$ 0.001\\
 5 & MCG~6-18-009 & 8.803 $\pm$ 0.005 & 8.735 $\pm$ 0.002 & \ldots & \ldots & 0.657 $\pm$ 0.003\\
 6 & MK~1212 & 8.740 $\pm$ 0.017 & 8.738 $\pm$ 0.005 & \ldots & \ldots & $-$0.322 $\pm$ 0.005\\
 8 & NGC~2532 & 8.763 $\pm$ 0.024 & 8.663 $\pm$ 0.017 & 8.722 $\pm$ 0.025 & $-$0.084 $\pm$ 0.017 & $-$0.037 $\pm$ 0.011\\
 9 & UGC~4261 & 8.534 $\pm$ 0.002 & 8.560 $\pm$ 0.002 & \ldots & \ldots & 0.058 $\pm$ 0.002\\
 10 & NGC~2535 & 8.874 $\pm$ 0.024 & 8.653 $\pm$ 0.004 & 8.656 $\pm$ 0.027 & 9.004 $\pm$ 0.009 & $-$0.871 $\pm$ 0.002\\
 11 & NGC~2543 & 8.770 $\pm$ 0.006 & 8.701 $\pm$ 0.003 & \ldots & \ldots & $-$0.865 $\pm$ 0.003\\
 12 & NGC~2537 & 8.613 $\pm$ 0.027 & 8.609 $\pm$ 0.023 & 8.714 $\pm$ 0.028 & 8.962 $\pm$ 0.023 & $-$3.264 $\pm$ 0.012\\
 13 & IC~2233 & 8.167 $\pm$ 0.003 & 8.213 $\pm$ 0.005 & \ldots & \ldots & $-$2.397 $\pm$ 0.003\\
\hline
	\end{tabular}
		\end{center}
	\end{minipage}
\hfill
     \begin{minipage}{92mm}
\caption{Host galaxy (non-nuclear) metallicities of the non-star-forming SFRS galaxies with available long-slit spectroscopy The nuclear component is subtracted similarly to the SFG host-galaxy metallicities. The full version of Table \ref{non-HII-Z} is available online from MNRAS.} 
\label{non-HII-Z}
	\begin{tabular}{@{}ccccc}
	
	\hline
	SFRS & Galaxy & \multicolumn{2}{c}{Host Galaxy Metallicity} & Classification \\
	\multicolumn{2}{c}{} & O3N2 & N2 \\ 
	\hline
	3 & NGC~2500 & 8.789 $\pm$ 0.033 & 8.914 $\pm$ 0.033 & LINER \\
	36 & IRAS~08572+3915NW & 8.716 $\pm$ 0.025 & 8.905 $\pm$ 0.013 & TO \\
	42 & IC~2434 & 8.755 $\pm$ 0.024 & 8.891 $\pm$ 0.017 & TO \\
	47 & NGC~2824 & 8.689 $\pm$ 0.032 & 8.924 $\pm$ 0.015 & LINER \\
	51 & IRAS~09197+2210 & 8.719 $\pm$ 0.071 & 8.895 $\pm$ 0.032 & TO \\
	61 & CGCG~181-068 & 8.676 $\pm$ 0.058 & 8.885 $\pm$ 0.021 & TO \\
	62 & NGC~2936 & 8.669 $\pm$ 0.052 & 8.714 $\pm$ 0.033 & LINER \\
	79 & IRAS~10120+1653 & 8.743 $\pm$ 0.064 & 8.891 $\pm$ 0.029 & LINER \\
	117 & IRAS~11102+3026 & 8.523 $\pm$ 0.241 & 8.960 $\pm$ 0.044 & Sy \\
	108 & IRAS~10565+2448W & 8.761 $\pm$ 0.012 & 9.031 $\pm$ 0.003 & Sy \\
	\hline
\end{tabular}

\end{minipage}



\end{table}
	

\begin{table}
	\vspace{10mm}
%	\hspace{-8mm}
	\begin{minipage}{242mm}
%			\begin{footnotetsize}

			
			\caption{Basic parameters and metallicity gradients for 12 galaxies of the SFRS. Column (1) SFRS Index; Column (2) Galaxy name; Column (3) Morphological types obtained from NED; Column (4) D25 angular diameters taken from Ashby et al.; Column (5) Distances in Mpc taken from Ashby et al.; Column (6) Activity classifications based on the nuclear spectra of galaxies. Columns (7) - (8) Circumnuclear and integrated slit Oxygen abundances, measured from calibration described in equation (\ref{eq:N2l}); Column (9) Central abundance (at radius r = 0) based on the derived N2 abundance gradient; Column (10) Characteristic abundance at radius r = 0.4$R_{25}$ based on the N2 derived abundance gradient; Column (11) Slope of the N2 abundance gradient. Column (12) Central abundance (at radius r = 0) based on the derived O3N2 abundance gradient; Column (13) Characteristic abundance at radius r = 0.4$R_{25}$ based on the 03N2 derived abundance gradient; Column (14) Slope of the 03N2 abundance gradient. The full version of Table \ref{z-grad} is available online from MNRAS.}
			\label{z-grad}
			\begin{tabular}{@{}cccccccccccccc}
				\hline
				SFRS & Galaxy & Morphology & D25 & Distance & Class & \multicolumn{2}{c}{12 + log(O/H)} & N2 & N2 & N2 Gradient & O3N2 & O3N2 & O3N2 Gradient \\
				&  & & (arcmin) & (Mpc) &  & (Nucleus) & (Integrated) & at r = 0 & at r = 0.4$R_{25}$ & (dex $R_{25}^{-1}$) & at r = 0 & at r = $0.4 R_{25}$ & (dex $R_{25}^{-1}$) \\
				(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14)  \\
				\hline
				8 & NGC~2532 & SAB(rs)c & 2.2 & 77.6 & H\,{\sc ii} & 8.76 (8.66) & 8.72 (8.94) &  8.662 $\pm$ 0.003 & 8.608 $\pm$ 0.004 & $-$0.12 $\pm$ 0.01 & 8.81 $\pm$ 0.01 & 8.66 $\pm$ 0.01 & $-$0.35 $\pm$ 0.03 \\
				41 & NGC~2750 & SABc & 2.2 & 37.0 & H\,{\sc ii} & 8.83 (8.68) & 8.74 (9.04) & 8.663 $\pm$ 0.003 & 8.69 $\pm$ 0.02 & 0.07 $\pm$ 0.04 & 8.81 $\pm$ 0.01 & 8.64 $\pm$ 0.03 & $-$0.39 $\pm$ 0.07 \\
				55 & NGC~2893 & (R)SB0/a & 1.1 & 24.0 & H\,{\sc ii} & 8.85 (8.75) & 8.72 (8.95) & 8.783 $\pm$ 0.003 & 8.80 $\pm$ 0.01 &	0.09 $\pm$ 0.04 & 8.89 $\pm$ 0.01 &	8.85 $\pm$ 0.02 & $-$0.15 $\pm$ 0.08 \\  
				129 & NGC~3686 & SB(s)bc & 3.2 & 21.0 & H\,{\sc ii} & 8.81 (8.62) & 8.75 (9.02) & 8.611 $\pm$ 0.002 & 8.69 $\pm$ 0.02 & 0.12 $\pm$ 0.03 & 8.81 $\pm$ 0.01 &	8.52 $\pm$ 0.05 &	$-$0.46 $\pm$ 0.08 \\  
				137 & NGC~3729 & SB(r)apec & 2.8 & 17.1 & H\,{\sc ii} & 8.63 (8.76) & 8.79 (8.99) & 8.745 $\pm$ 0.002 & 8.82 $\pm$ 0.02 & 0.14 $\pm$ 0.04 & 8.612 $\pm$ 0.004 & 8.81 $\pm$ 0.06 & 0.36 $\pm$ 0.11 \\
				147 & NGC~3811 & SB(r)cd? & 2.2 & 54.2 & H\,{\sc ii} & 8.74 (8.67) & 8.72 (8.93) & 8.675 $\pm$ 0.005 & 8.63 $\pm$ 0.01 & $-$0.11 $\pm$ 0.03 & 8.77 $\pm$ 0.01 & 8.62 $\pm$ 0.03 & $-$0.33 $\pm$ 0.06 \\  
				148 & NGC~3822 & S0? & 1.4 & 94.6 & Sy &  \ldots & 8.86 (8.97) & \ldots & 8.67 $\pm$ 0.01 & 0.03 $\pm$ 0.02 &	\ldots & 8.69 $\pm$ 0.02 & 0.38 $\pm$ 0.06 \\  
				163 & NGC~4014 & S0/a & 2.2 & 62.6 & H\,{\sc ii} & 8.67 (8.76) & 8.79 (8.90) & 8.723 $\pm$ 0.009 & 8.61 $\pm$ 0.03 & $-$0.25 $\pm$ 0.06 & 8.70 $\pm$ 0.02 & 8.65 $\pm$ 0.07 &	$-$0.11 $\pm$ 0.15 \\  
				178 & NGC~4162 & (R)SA(rs)bc & 2.3 & 42.5 & H\,{\sc ii} & 8.67 (8.75) & 8.74 (8.89) & 8.730 $\pm$ 0.007 &	8.65 $\pm$ 0.01 & $-$0.17 $\pm$ 0.02 & 8.68 $\pm$ 0.01 & 8.65 $\pm$ 0.02 &	$-$0.07 $\pm$ 0.03 \\  
				186 & NGC~4234 & (R')SB(s)m & 1.3 & 30.0 & H\,{\sc ii} & 8.61 (8.56) & 8.86 (9.09) & 8.558 $\pm$ 0.002 &	8.585 $\pm$ 0.002 &	0.10 $\pm$ 0.01 & 8.61 $\pm$ 0.002 & 8.649 $\pm$ 0.003 & 0.154 $\pm$ 0.01 \\
				218 & NGC~4625 & SAB(rs)mpec & 2.2 & 9.2 & H\,{\sc ii} & 8.69 (8.69) & 8.75 (8.88) & 8.680 $\pm$ 0.007 &	8.64 $\pm$ 0.02 &	$-$0.08 $\pm$ 0.04 & 8.72 $\pm$ 0.02 & 8.67 $\pm$ 0.05 &	$-$0.10 $\pm$ 0.11 \\
				316 & NGC~5660 & SAB(rs)c & 2.8 & 38.9 & H\,{\sc ii} & 8.75 (8.67) & 8.73 (8.95) & 8.680 $\pm$ 0.002 & 8.56 $\pm$ 0.01 & $-$0.21 $\pm$ 0.01 & 8.77 $\pm$ 0.01 & 8.55 $\pm$ 0.01 & $-$0.39 $\pm$ 0.02 \\  
				\hline
			\end{tabular}

			

%	\end{footnotetsize}
	\end{minipage}

\end{table}

\end{landscape}

